GraphGPT: Graph Instruction Tuning for Large Language Models

Graph Neural Networks (GNNs) have evolved to understand graph structures through recursive exchanges and aggregations among nodes. To enhance robustness, self-supervised learning (SSL) has become a vital tool for data augmentation. Traditional methods often depend on fine-tuning with task-specific labels, limiting their effectiveness when labeled data is scarce. Our research tackles this by advancing graph model generalization in zero-shot learning environments. Inspired by the success of large language models (LLMs), we aim to create a graph-oriented LLM capable of exceptional generalization across various datasets and tasks without relying on downstream graph data. We introduce the GraphGPT framework, which integrates LLMs with graph structural knowledge through graph instruction tuning. This framework includes a text-graph grounding component to link textual and graph structures and a dual-stage instruction tuning approach with a lightweight graph-text alignment projector. These innovations allow LLMs to comprehend complex graph structures and enhance adaptability across diverse datasets and tasks. Our framework demonstrates superior generalization in both supervised and zero-shot graph learning tasks, surpassing existing benchmarks. The open-sourced model implementation of our GraphGPT is available at https://github.com/HKUDS/GraphGPT.

==> model_back.tex <==
\section{Preliminaries}
\label{sec:relate}
In this section, we present preliminaries and common definitions in this work, 
and then formalize the precise problems of traffic prediction.
Notations frequently used in this paper are demonstrated in Appendix Table~\ref{tab:notations}.


% \subsection{Multi-grained Geographical Region}


\begin{Dfn}
    \label{dfn:mlti}
\textbf{Multi-grained Geographical Region}. 
% According to the paradigm of traffic flow prediction, 
We partition the whole city into $M\times N$ (in total $R$) disjoint regions, which is a fine-grained region-level division.
Moreover, we divide the urban into $ \frac{M}{\lambda_{d}}\times \frac{N}{\mu_{d}}$ (in total $D$) and $ \frac{M}{\lambda_{z}}\times \frac{N}{\mu_{z}}$ (in total $Z$),
where the $1 \le\lambda_{d}\le M$, $1 \le \mu_{d}\le N$ are mid-grained district-level scale factors and $1 \le \lambda_{z} \le M$, $1 \le \mu_{z}\le N$ are coarse-grained zone-level scale factors, respectively.
($\lambda_z \geq \lambda_d$, $\mu_z\geq \mu_d$, to satisfy the multi-grained definition.) 

\end{Dfn}
% The detailed implementation of the scale operation is mean-pooling proposed in Section~\ref{sec:hgsl}. 

\begin{Dfn}
    \textbf{The Entire and Windowed Traffic Flow Data}. 
    % We divide traffic flow data into two categories, the whole and windowed traffic flow data.
    The entire data is divided into multiple granularities as described in Definition~\ref{dfn:mlti}, which is mathematically described as 
    $\textbf{X}^{\mathcal{R}}\in\mathbb{R}^{R\times \mathcal{T}\times F}$, $\textbf{X}^{\mathcal{D}}\in\mathbb{R}^{D\times \mathcal{T}\times F}$ and $\textbf{X}^{\mathcal{Z}}\in\mathbb{R}^{Z\times \mathcal{T}\times F}$ ($R\geq D \geq Z$), 
    where $R$, $D$, $Z$ denote the number of multi-grained spatial units, $\mathcal{T}$ presents all time slots for data recording, and $F=2$ is the number of features, i.e., inflow and outflow.
    As to windowed traffic flow data is a three-way tensor $\textbf{X}\in\mathbb{R}^{R\times T\times F}$, which is split from the entire data with a moving time window.
    % Generally, the entire and windowed traffic flow data serve the task of hypergraph structure learning and traffic prediction, respectively.
    

\end{Dfn}

\begin{Dfn}
    \textbf{External Factors}. 
    Four categories of external factors are taken into account in ST-HGformer, that is timestamps, holidays, weather conditions and temperatures.
    % Regarding timestamps and holidays, we adopt One-Hot Encoding to encode hour-of-day, day-of-week, week-of-month and holiday temporal information into binary vectors $v^{(h-d)}$, $v^{(d-w)}$, $v^{(w-m)}$ and $v^{(h)}$ respectively.
    % Concerning weather conditions, such as rainfall, snowfall, etc., we employ the aforementioned strategy to generate the binary vector $v^{(w)}$.
    % Furthermore, we linearly normalize the temperatures so that its range is controlled between [0-1] and encode the similar binary vector $v^{(t)}$.
    For every time slot, we concatenate binary vectors according to the external information and obtain the external factor at the $i^{th}$ time interval $E_i^{(\varepsilon)} = v^{(h-d)}||v^{(d-w)}||v^{(w-m)}||v^{(h)}||v^{(w)}||v^{(t)}\in \mathbb{R}^{\epsilon}$, 
    where $\epsilon$ is the external dimension, 
    $v^{(h-d)}$, $v^{(d-w)}$, $v^{(w-m)}$, $v^{(h)}$ are hour-of-day, day-of-week, week-of-month, holiday encoded temporal binary vectors, 
    $v^{(w)}$ denotes the weather condition binary vector, $v^{(t)}$ is the temperature vector.
\end{Dfn}

\noindent\textbf{Problem Statement}.
With the above definitions, the traffic flow prediction is expressed as that:
\noindent\textbf{Input}:
traffic flow tensor $X=\{X_{:, t-T, :},\cdots, X_{:, t-1, :}\}\in \mathbb{R}^{R\times T\times F}$, 
historical external factor tensor $E^{(\varepsilon)}=\{E^{(\varepsilon)}_{t-T},\cdots, E^{(\varepsilon)}_{t-1}\}\in \mathbb{R}^{T\times \epsilon}$, 
and the external factor tensor $E^{(\varepsilon)}_{t}$ at the target time slot $t$. 
\noindent\textbf{Output}: a predictive function $f$ to infer the traffic flow tensor at the target time slot $t$ $X_{:, t, :}$, which is formulized as the equation: 
$X_{:, t, :} = f(X, E^{(\varepsilon)}, E^{(\varepsilon)}_{t})$.

% \subsection{External Factors}
% \subsection{Problem Statement}



==> solution_back.tex <==
\section{Methodology}
\label{sec:solution}
\begin{figure}[h]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    %\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
    \vspace{-3.5mm}
    \includegraphics[width=0.47\textwidth]{imag/over_new.pdf}
    \end{center}
    \vspace{-3mm}
    \caption{Overview of \model\ . (a) The workflow of our \model\ framework. 
    (b) The data categorie introduced in preliminaries and data processing method before training. 
    (c) Diagram of the input and output of the hypergraph structure learning module.
    (d) The diffusion-enhanced mask construction method for simplified implementation of diffusion temporal hypergraph convolutions.
    }
    \label{fig:overall}
    \vspace{-4mm}
\end{figure}
In this section, we present detailed descriptions of different components of the proposed \model\ . 
The overall architecture of \model\ is illustrated in Figure~\ref{fig:overall}.



\subsection{Hypergraph Structure Learning\label{sec:hgsl}}

To comprehensively explore the global spatial correlations of traffic flow data and obtain the attention mask required by the transformer, 
we employ the idea of graph structure learning to construct the hypergraph adjacency matrix. 
The workflow of Hypergraph Structure Learning (HGSL) is demonstrated in Appendix Figure~\ref{fig:hgsl}.



% Mathematically, let $\mathbf{X}_{\mathcal{R}}\in \mathbb{R}^{R\times \mathcal{T}\times F}$ be the whole traffic data, where $R$ denotes the number of regions in a city and $\mathcal{T}$ denotes the total time steps the data contains, 
% and $\mathbf{\Phi}\in \mathbb{R}^{R\times E}$ be the binary hypergraph adjacency, where $E$ presents the number of hyperedges in the hypergraph. 

% Primarily, we formulize the hypergraph structure learning into learning a Function $\mathbf{G}_{HG}: \mathbf{\Phi} = \mathbf{G}_{HG}(\mathbf{X}_{\mathcal{R}})$.
Motivated by the recent success of graph structure learning applied in various fields\cite{SLAPS, LDS, GTS}, 
we propose a double-view and multi-grained hypergraph structure learning method by encoding the spatial-temporal traffic flow data into double-view (inflow and outflow) graph embeddings and utilize the attentive score function to measure the latent global correlations between region-district pairs and region-zone pairs.

Especially, \model\  firstly scales the spatial size of the region-level traffic flow data the mean-pool, which is defined as follows:
\begin{align}
	\mathbf{X}^{\mathcal{D}\backslash \mathcal{Z}} = \text{Mean-Pooling}_{\mathcal{D}\backslash Z}(\mathbf{X}^{\mathcal{R}})\label{eq1}
\end{align}
% \begin{equation}
% 	\mathbf{X}_{\mathcal{Z}} = \mathbf{Pooling}_{R\mathcal{Z}}(\mathbf{X}_{\mathcal{R}})\label{eq2}
% \end{equation}
where $\mathbf{X}^{\mathcal{R}}\in\mathbb{R}^{R\times \mathcal{T}\times F}$, $\mathbf{X}^{\mathcal{D}}\in\mathbb{R}^{D\times \mathcal{T}\times F}$ and $\mathbf{X}^{\mathcal{Z}}\in\mathbb{R}^{D\times \mathcal{T}\times F}$ present the Region-, District- and Zone-level data respectively, 
as well as $\text{Mean-Pooling}_{\mathcal{D}}(\cdot)$ and $\text{Mean-Pooling}_{\mathcal{Z}}(\cdot)$ denote the mean-pooling.
Then, we employ Multilayer Perceptron (MLP) to extract traffic inflow- and outflow-features at different levels, as is formulized as follows:
\begin{equation}
	\mathbf{Z}_{:, :, i (o)}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}} = \text{MLP}(\mathbf{X}_{:, :, i (o)}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}})\label{eq3}
\end{equation}
% \begin{equation}
% 	\mathbf{Z}_{r\backslash d\backslash z, :, o} = \mathbf{MLP}(\mathbf{X}_{r\backslash d\backslash z, :, o})\label{eq4}
% \end{equation}
where $\mathbf{X}_{:, :, i}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}}$, $\mathbf{X}_{:, :, o}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}}\in \mathbb{R}^{R\backslash D\backslash Z \times \mathcal{T}}$ denote raw region-$\backslash$ district-$\backslash$ zone-data from inflow- and outflow-view, 
as well as $\mathbf{Z}_{:, :, i}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}}$, $\mathbf{Z}_{:, :, o}^{\mathcal{R}\backslash \mathcal{D}\backslash \mathcal{Z}}\in \mathbb{R}^{R\backslash D\backslash Z \times \mathcal{T}^{\prime}}$ present extracted region-$\backslash$ district-$\backslash$ zone-data from inflow- and outflow-view.
After feature extracting, we calculate region-district and region-district correlation score, that is $\theta^{\mathcal{D}}$ and $\theta^{\mathcal{Z}}$ as follows:
\begin{align}
	\theta^{\mathcal{D}\backslash \mathcal{Z}} &= \mathbf{FC}(\mathbf{FC}(score^{\mathcal{D}\backslash \mathcal{Z}}_{i}||score^{\mathcal{D}\backslash \mathcal{Z}}_{o})) \nonumber \\ 
	score^{\mathcal{D}\backslash \mathcal{Z}}_{i (o)} &= \text{Flatten}((\mathbf{Z}_{:, :, i (o)}^{\mathcal{R}})\cdot (\mathbf{Z}_{:, :, i (o)}^{\mathcal{D}\backslash \mathcal{Z}})^\top)\label{eq6}
\end{align}  
% \begin{equation}
% 	score^{\mathcal{D}\backslash \mathcal{Z}}_{i (o)} = \text{Flatten}((\mathbf{Z}_{:, :, i (o)}^{\mathcal{R}})\cdot (\mathbf{Z}_{:, :, i (o)}^{\mathcal{D}\backslash \mathcal{Z}})^\top)\label{eq6}
% \end{equation}
where $score^{\mathcal{D}}_{i (o)} \in \mathbb{R}^{(R*D)}$, $score^{\mathcal{Z}}_{i (o)} \in \mathbb{R}^{(R*Z)}$, $\theta^{\mathcal{D}} \in \mathbb{R}^{(R*D)\times 2}$, $\theta^{\mathcal{Z}} \in \mathbb{R}^{(R*Z)\times 2}$, as well as $\mathbf{FC}$ and $\text{Flatten}$ denote fully connected and flatten layers.  

To obtain a discrete structure $\mathbf{\Phi}$ that serves as the transformer mask, we employ the Gumbel-Softmax reparametrization trick inspired by\cite{softmax_1, softmax_2}:
\begin{equation}
	\mathbf{\Phi}^{\mathcal{D}\backslash \mathcal{Z}} = \text{GumbelSoftmax}((\theta^{\mathcal{D}\backslash \mathcal{Z}}+\textsl{g})/\tau)\label{eq7}
\end{equation}
where $\textsl{g}$ denotes a vector of i.i.d. samples drawn from a Gumbel(0,1) distribution and $\tau$ is the temperature controlling the smoothness of the distribution.
Note that to apply the learned structure in the undermentioned hypergraph transformer, the $\mathbf{\Phi}^{\mathcal{D}\backslash \mathcal{Z}}$ is reshaped to $\mathbb{R}^{R\times D\backslash Z}$, where $D$ and $Z$ denote the number of districts and zones, i.e., the number of hyperedges.

To sum up, through multi-grained traffic views in the urban, we construct hypergraph where the nodes are different regions in the urban with the number of $R$,
and hyperedges are abstract districts and zones with the number of $D$ and $Z$.


% \subsection{Spatial Encoder}
% In this subsection, we propose spatial encoder to capture the local and global spatial dependencies, with 2D convolution resnet and well designed hypergraph transformer.

\subsection{Local Spatial Dependencies Modeling}
In this subsection, we introduce our proposed methods to model the local dependencies with numerous external factors.
% \subsubsection{External Factors Fusion}
% External factors, such as timestamps, holidays, weather conditions, etc., contain rich semantic information about the city, which affects the changing regularities of traffic flow.
% Consequently, we aggregate historical traffic data features and external factor features at the beginning of \model\ , 
% and fuse the target external factor features at the end of \model\ .
% Primarily, we exploit 2-D convolution and Multilayer Perceptron (MLP) to reshape the historical traffic flow tensor and external factors for fusing, which is defined as follows:
% \begin{equation}
% 	E_{pre}^{(r)} = \text{2D-Conv}(X)+\text{MLP}(E^{(e)})\label{eq:fusin}
% \end{equation}
% where $X\in \mathbb{R}^{R\times T\times F}$ denotes the traffic tensor, $E^{(e)} \in \mathbb{R}^{T\times \epsilon}$ presents the external factor tensor and $E_{pre}\in \mathbb{R}^{R\times T\times F^{\prime}}$ serves as the pre-encoded feature.
% Particularly, $\text{2D-Conv}$ is formulized as follows:
% \begin{equation}
% 	E_{(conv)} = \sigma(W_{(conv)}*X+b_{(conv)})\label{eq:conv}
% \end{equation}
% where $W_{(conv)}$ and $b_{(conv)}$ present weight and bias parameters, $\sigma$ is an activation function.
% Concerning the fusion of target external factors, we introduce in Section~\ref{sec:final}.
Before modeling local spatial dynamics, we aggregate historical traffic data features and external factor features (\eg, timestamps, holidays, weather conditions, etc.) at the beginning of \model\ .
Specifically, we exploit 2-D convolution and Multilayer Perceptron (MLP) to project traffic data $X\in \mathbb{R}^{R\times T\times F}$ and external factor $E^{(\varepsilon)}\in \mathbb{R}^{T\times \epsilon}$ into the same space and obtain the pre-processed embedding $E^{(0)}\in \mathbb{R}^{R\times T\times F^{\prime}}$. 
Concerning the fusion of target external factors, we introduce in Section~\ref{sec:final}.

% \subsubsection{2D Convolution Resnet}
For local spatial dependencies modeling, as is well known, one region's traffic patterns are also affected by other ones around it, which we call local correlation. 
Actually, manifold previous work have made excellent explorations in capturing local dependencies of urban traffic flow, whether graph-based or grid-based.
For our grid-based task, we take a widely proven 2D convolution residual network approach to tackle the problem of local dependencies modeling~\cite{ST-ResNet}.
More particularly, we formulize 2D convolution resnet as shown in the equation below:
\begin{align}
	E_{l+1} &= \text{2D-Conv}_{l}(E_{l})+E_{l}\nonumber \\
	\text{2D-Conv}(X) &= \sigma(W^{(conv)}*X+b^{(conv)})\label{eq:conv}
\end{align}
% \begin{equation}
% 	\text{2D-Conv}(X) = \sigma(W^{(conv)}*X+b^{(conv)})\label{eq:conv}
% \end{equation}
where $l=[1,L]$ is the index of layers and $L$ is the maximum number of layers, $E_1 = E^{(0)}$, as well as the definition of $\text{2D-Conv}_{l}$ is demonstrated in Eq.~\eqref{eq:conv}.
% Eventually, we employ the $\text{2D-Conv}$ as Eq.~\eqref{eq:conv} to reshape the output of resnet in Eq.~\eqref{eq:res}, which is shown as follows:
% \begin{equation}
% 	E^{(r)} = \text{2D-Conv}_{end}(E_{L+1}^{(r)})\label{eq:endconv}
% \end{equation}
And output of 2D convolution resnet $E^{(\alpha)}\in \mathbb{R}^{R\times T\times d}$ is the final embeddings in local spatial dependencies modeling, and $d$ is the transformer dimension. 
We employ the 2D convolutions with \emph{kernel}=3, \emph{stride}=1,  \emph{padding}=1 to enhance the capability of local dependencies modeling in this module.

\subsection{Hypergraph Transformer}
Previous work, whether GNN or CNN, has focused on modeling local dependencies, but global dependencies also play a non-negligible role in traffic flow prediction.
In particular, traffic patterns in various regions of the city that have similar urban functionality (e.g., the similar POI information) are highly correlated. 
Meanwhile, urban functionality can be abstracted into multiple granularities, i.e., low-coarse-grained for district-level (e.g., different administrative districts in the cities) and high-coarse-grained for zone-level (e.g., residential zones, commercial zones).
Therefore, inspired by recent achievements of transformer especially for hypergraph~\cite{HGformer_Res}, we propose a multi-grained hypergraph transformer framework utilizing head-aware Multi-head Attention, to encode head- and hyperedge-specific graph embeddings leveraging multi-grained geographical information extracted from hypergraph structure learning. 

\subsubsection{Node-Edge Multi-head Attention\label{subsec: node2edge}}
To begin with, we employ the head-aware Node-Edge Multi-head Attention to encode region-level node embeddings $E^{(\alpha)}$ into multi-grained level hyperedge embeddings $E^{(d\backslash z)}$, which is formulized as follows:
\begin{equation}
	E^{(d\backslash z)} = \text{Node2Edge-MultiHead}(Q,K,V) = ||_{i}^{H}head_iW_{O}\label{eq8}
\end{equation}
where $E^{(d\backslash z)}\in \mathbb{R}^{D\backslash Z\times T\times d}$ denotes the edge embeddings, $H$ presents the number of head, $W_{O}\in \mathbb{R}^{d\times d}$ is the parameter matrices for projection, 
as well as $Q$, $K$ and $V$ serve as query, key and value respectively in the conventional transformer paradigm. 
In detail, head-aware $head_i$ is defined as follows:
\begin{equation}
    \begin{split}
        head_i &= \text{Node2Edge-Attention}(Q,K,V)\\
        &=c_{i,:}\odot((\text{Softmax}(\frac{QK^T}{\sqrt{d_k}}\odot\mathbf{\Phi}_{r-d\backslash z}))V)\label{eq9}
    \end{split}
\end{equation}
where query $Q=Z\in\mathbb{R}^{D\backslash Z\times\frac{d}{H}}$, key $K=E^{(\alpha)}W_k\in\mathbb{R}^{R\times\frac{d}{H}}$, 
value $V=E^{(\alpha)}W_v\in\mathbb{R}^{R\times\frac{d}{H}}$, head-aware category $c\in\mathbb{R}^{H\times D\backslash Z}$ motivated by ~\cite{GroupNet}, 
$\odot$ denotes element-wise product, and $\mathbf{\Phi}^{\mathcal{D}\backslash \mathcal{Z}}$ presents aforementioned learned hypergraph structure in Section~\ref{sec:hgsl}.
We argue that learned discrete hypergraph structure could adaptively drop the task-irrelative global interactions. 
As for head-aware category, we adopt the similar Gumbel reparametrization trick as Section~\ref{sec:hgsl} to compute, which is particularly defined as follows:
\begin{align}
	c_{:,i} &= \text{Softmax} ((\text{MLP}(z_i) + \textsl{g})/\tau)\in \mathbb{R}^{H}\nonumber \\ 
	z_i &=\sum_{E_j^{(\alpha)}\in e_i}w_jE_j^{(\alpha)} \nonumber\\
	w_j &=\text{MLP} (E_j^{(\alpha)}||\sum_{E_m^{(\alpha)}\in e_i}E_m^{(\alpha)}) \label{eq12}
\end{align}

% \begin{equation}
%     z_i=\sum_{E_j^{(\alpha)}\in e_i}w_jE_j^{(\alpha)} \label{eq11}
% \end{equation}
% \begin{equation}
%     w_j =\text{MLP} (E_j^{(\alpha)}||\sum_{E_m^{(\alpha)}\in e_i}E_m^{(\alpha)}) \label{eq12}
% \end{equation}
where $e_i = \text{Hyper-Neighbor}(E_i^{(\alpha)})$. 
As we all know, there are various POI (Point of Interests) types(e.g., Residential, Education Facility, Cultural Facility and other 10 categories in NYC),
and we argue that head-aware category $c$ is able to adaptively learn the latent POI-like distribution of diverse edges in different heads message passing processes.

\subsubsection{Cross-Hyperedge Graph Convolution}
To extract features adequately and enhance the message passing in edge-level, we adopt the Cross-Hyperedge Graph Convolution Networks (CHE-GCN), which is formulized as follows:
\begin{align}
    \hat{E}^{(d\backslash z)} &= \text{CHE-GCN}(E^{(d\backslash z)}) \nonumber\\
    &=\mathbf{LeakyReLU}(\mathbf{\Psi}^{\mathcal{D}\backslash \mathcal{Z}} \cdot E^{(d\backslash z)} + E^{(d\backslash z)}) \nonumber\\
    \mathbf{\Psi}^{\mathcal{D}\backslash \mathcal{Z}} &= \text{Softmax}(\mathbf{ReLU}(\mathcal{E}^{(d\backslash z)}\mathcal{E}^{(d\backslash z)\top})) \label{eq14}
\end{align}
% \begin{equation}
%     \mathbf{\Psi}^{\mathcal{D}\backslash \mathcal{Z}} = \text{Softmax}(\mathbf{ReLU}(\mathcal{E}^{(d\backslash z)}\mathcal{E}^{(d\backslash z)\top})) \label{eq14}
% \end{equation}
where $\hat{E}^{(d\backslash z)}, E^{(d\backslash z)}\in \mathbb{R}^{D \backslash Z\times T \times d }$ denote multi-grained embeddings after and before encoding, 
$\mathbf{\Psi}^{\mathcal{D}\backslash \mathcal{Z}} \in \mathbb{R}^{D \backslash Z\times D \backslash Z}$ presents the hyperedge adjacency matrix, 
$\mathcal{E}^{(d\backslash z)}$ is the hyperedge embeddings for learning $\mathbf{\Psi}^{\mathcal{D}\backslash \mathcal{Z}}$ adaptively with the random initialization, 
$\mathbf{LeakyReLU}$ and $\mathbf{ReLU}$ are nonlinear activation functions.

\subsubsection{Edge-Node Multi-head Attention}
Resembling general hypergraph neural networks, our framework also exploits edge-to-node message passing progress, which is similar to hypergraph self-attention in Section~\ref{subsec: node2edge}.
More particularly, Edge-Node Multi-head Attention is declared as follows:
\begin{equation}
    \tilde{E}^{(d\backslash z)} = \text{Edge2Node-MultiHead}(Q^{\prime},K^{\prime},V^{\prime}) = ||_{i}^{H}head_i^{\prime}W_{O}^{\prime} \label{eq15}
\end{equation}
where $\tilde{E}^{(d\backslash z)}\in \mathbb{R}^{}$ indicates the multi-grained region embeddings after encoding. 
As to $head_i^{\prime}$, we take simplified implementation for the reduction of parameters and calculation complexity, which is defined as follows:
\begin{equation}
    \begin{split}
        head_i^{\prime} &= \text{Edge2Node-Attention}(Q,K,V)\\
        &=(\mathbf{Softmax}(\frac{Q^{\prime}K^{\prime T}}{\sqrt{d_{k^{\prime}}}}))V^{\prime}\label{eq16}
    \end{split}
\end{equation}
where query $Q^{\prime}=K\in\mathbb{R}^{R\times\frac{d}{H}}$, key $K^{\prime}=Q \in\mathbb{R}^{D\backslash Z\times\frac{d}{H}}$, 
value $V=\hat{E}^{(d\backslash z)}\in \mathbb{R}^{R\times T\times d}$.

\subsubsection{Multi-Grained Fusion}
With encoded embeddings $\tilde{E}^{(d)}$ and $\tilde{E}^{(z)}$, we consider fusing multi-grained embeddings to aggregate multiple global correlations extracting from the whole city.
For detailed implementation, we employ the Fully Connected Layer as follows:
\begin{equation}
    E^{(\beta)} = \mathbf{FC}(\tilde{E}^{(d)}||\tilde{E}^{(z)}) \label{eq17}
\end{equation}
where $E^{(\beta)}\in \mathbb{R}^{R\times T\times d}$ denotes the final encoded embeddings by hypergraph transformer, and $||$ denotes the concatenate operation.

% \subsection{Temporal Encoder}

\subsection{Diffusion Temporal Hypergraph Convolution Layer}
The traffic datasets in this work are derived from the preprocessing of bicycle or taxi trip datasets, 
which purely contain start and end station latitude and longitude, yet no latitude and longitude of the trajectory pathway.
Thus, we call it trajectory-agnostic data.
And we argue that mining the latent trajectories of the trajectory-agnostic data enables more comprehensive temporal dependencies modeling, so as to achieve increasingly accurate traffic flow prediction.
To this end, we propose a trajectory-aware method, i.e., diffusion temporal hypergraph convolution layer, 
to simulate the diffuse nature of traffic flow feature maps at different time slots between regions caused by the trajectory of the agent (e.g., bike and taxi in this paper) with temporal continuity.
And more detailed formulization is as follows:
\begin{equation}
    E^{(\gamma)}_{(t-p)\sim (t-1)} = \sigma(\mathbf{\Omega}^{\mathbf{T}}\cdot \sigma (\mathbf{\Omega}\cdot E^{(\beta)}_{(t-p)\sim (t-1)})) \label{eq:thgcn}
\end{equation}
where $E^{(\beta)}_{(t-p)\sim (t-1)} = ||_{i=t-p}^{t-1}E^{(\beta)}_i\in \mathbb{R}^{pR\times d}$ is timeblock tensor stacked in dimension 0 with $E^{(\beta)}$ from time slot $t-p$ to $t-1$, $p$ is the length of the diffusion timeblock, $\sigma$ denotes activation function.
While $\mathbf{\Omega}\in \mathbb{R}^{E_p\times pR}$ is a learnable temporal diffusion hypergraph adjacency matrix and $E_p$ is the number of hyperedges in a single timeblock.
Specifically speaking, we construct temporal hypergraph where nodes denote the all regions in a timeblock with the number of $pR$ and hyperedges, 
with the number of $E_p$, connect the nodes that satisfy the region-wise characteristics of diffusion. 
We assume that hyperedges are able to explore diffusion relationships between continuous time slots of traffic flows.

% \noindent\textbf{Simplified Implementation with Diffusion-Enhanced Mask}
\noindent\textbf{Simplified Implementation}.
Obviously, the randomly initialized learnable hypergraph adjacency matrix $\mathbf{\Omega}$ is difficult to converge, allowing the hyperedges to connect different regions of temporal diffusion as we envision. 
Accordingly, we propose to add the diffusion-enhanced mask and implemented Eq.~\eqref{eq:thgcn}, which is formulized as follows:
\begin{equation}
    E^{(\gamma)}_{(t-p)\sim (t-1)} = \sigma(\mathbf{MASK}(\mathbf{\Omega}^{\mathbf{T}}\cdot \mathbf{\Omega})\cdot E^{(\beta)}_{(t-p)\sim (t-1)}) \label{eq:simp}
\end{equation}
where $\mathbf{\Omega}\in \mathbb{R}^{E_p\times pR}$ is learnable adjacency matrix and $\mathbf{MASK}$ denotes the diffusion-enhanced mask, which is compute as follows:
\begin{equation}
    \mathbf{MASK} = \text{Diff-Concat}(\mathbf{A}, \mathbf{A}^{2\eta }, \cdots, \mathbf{A}^{p\eta}) \label{eq:hadj}
\end{equation}
where $\text{Diff-Concat}$ presents the matrix concatenate way shown in the lower right corner (d) of Figure~\ref{fig:overall}, 
$\mathbf{A}$ is the pre-defined region adjacency matrix, and $\eta$ denotes diffusion factor that can be valued as $1,2,3\cdots$.
Finally, $E^{(\gamma)}_{(t-p)\sim (t-1)}$ is scaled from $\mathbb{R}^{(p*R)\times d}$ to $\mathbb{R}^{R\times d}$ with $\text{MLP}$.
% \begin{equation}
%     E^{(th)}_{(t-p)\sim (t-1)} = \text{MLP}(E^{(th)}_{(t-p)\sim (t-1)}) \label{eq:scale}
% \end{equation}
In general, timeblock window is sliding above $E^{(\beta)}\in \mathbb{R}^{R\times T\times d}$ with length $p$, thus generating the final output $E^{(\gamma)}\in \mathbb{R}^{R\times T^{\prime}\times d}$ and $T^{\prime} = T-p+1$. 
Compared with other temporal modeling approaches such as temporal convolutions, temporal hypergraph convolutions exploit the diffusion nature of traffic flow and have a superiority in interpretability which is shown in Section~\ref{sec:case}. 

\subsection{Temporal Transformer}
\label{sec:tformer}
The traffic transitional regularities are impacted not only by short-term temporal dependencies, but also by long-term temporal dependencies.
To capture long-term temporal correlations, we adopt temporal transformer, which is widely recognized for being good at modeling long-time sequences.
With the output $E^{(\gamma)} = \{E^{(\gamma)}_{:,i,:}\}_{i=1}^{T^{\prime}}$ of diffusion temporal hypergraph convolution layer, 
the formulization is demonstrated as follows:
\begin{equation}
    E^{(\rho)} = \text{Temporal-MultiHead}(Q^{\prime\prime},K^{\prime\prime},V^{\prime\prime}) = ||_{i}^{H}head_i W_{O}^{\prime\prime} \label{eq:tformer1}
\end{equation}
% \begin{equation}
%     head_i = \text{Temporal-Attention}(Q^{\prime\prime},K^{\prime\prime},V^{\prime\prime})\\
%         =\text{Softmax}(\frac{Q^{\prime\prime}K^{\prime\prime T}}{\sqrt{d_{k^{\prime\prime}}}})V^{\prime\prime} \label{eq:tformer2}
% \end{equation}
where query $Q^{\prime\prime} = \{E^{(\gamma)}_{:,i,:}\}_{i=1}^{T^{\prime}}W_Q^{\prime\prime} \in  \mathbb{R}^{T^{\prime}\times \frac{d}{H}}$, 
key $K^{\prime\prime} = \{E^{(\gamma)}_{:,i,:}\}_{i=1}^{T^{\prime}}W_K^{\prime\prime}\in  \mathbb{R}^{T^{\prime}\times \frac{d}{H}}$, 
value $V^{\prime\prime} = \{E^{(\gamma)}_{:,i,:}\}_{i=1}^{T^{\prime}}W_V^{\prime\prime}\in  \mathbb{R}^{T^{\prime}\times \frac{d}{H}}$, 
and $E^{(\gamma)}\in \mathbb{R}^{R\times T^{\prime} \times d}$ denotes the output of temporal transformer.

% And worth pointing out, we aggregate the external factors with

\subsection{Predictive and Learning Processes of \model\ }
\label{sec:final}
% In this subsection, we propose the predictive networks with the target external factors and the optimized objective of \model\ .

With transformer embeddings $E^{(\rho)}$ and the target external factors $E_t^{(\varepsilon)}$, we fuse them together and form the fusion embeddings into the shape of the ground-truth traffic flow tensor to obtain  predictive traffic flow $\hat{\mathbf{X}}_t\in \mathbb{R}^{R\times F}$.
% The formulization is described as follows:
% \begin{equation}
%     \hat{\mathbf{X}}_t = \sigma(\text{MLP}_1(E^{(\rho)}+\text{MLP}_2(E_t^{(\varepsilon)}))) \label{eq:fuse}
% \end{equation}
% where $\hat{\mathbf{X}}_t\in \mathbb{R}^{R\times F}$ is the predictive traffic flow and $\sigma$ denotes the activation function (e.g., $\tan (\cdot)$).
% \subsubsection{Optimized Objective}
In \model\ , we simultaneously predict the inflow and outflow traffic flow in each region across the whole urban and the loss function is formulized as below:
\begin{equation}
    \mathcal{L}=\sum_{r=0}^{R-1}[(\hat{\mathbf{X}}_{r,t,i}-\mathbf{X}_{r,t,i})^2-(\hat{\mathbf{X}}_{r,t,o}-\mathbf{X}_{r,t,o})^2] \label{eq:loss}
\end{equation}
where $\hat{\mathbf{X}}_{r,t,i}$ and $\hat{\mathbf{X}}_{r,t,o}$ denote the ground-truth the input and output traffic volume, at the $r^{th}$ region and $t^{th}$ time slot.



